ONER: Online Experience Replay for Incremental Anomaly Detection

Incremental anomaly detection aims to sequentially identify defects in industrial product lines but suffers from catastrophic forgetting, primarily due to knowledge overwriting during parameter updates and feature conflicts between tasks. In this work, We propose ONER (ONline Experience Replay), an end-to-end framework that addresses these issues by synergistically integrating two types of experience: (1) decomposed prompts, which dynamically generate image-conditioned prompts from reusable modules to retain prior knowledge thus prevent knowledge overwriting, and (2) semantic prototypes, which enforce separability in latent feature spaces at pixel and image levels to mitigate cross-task feature conflicts. Extensive experiments demonstrate the superiority of ONER, achieving state-of-the-art performance with +4.4% Pixel AUROC and +28.3% Pixel AUPR improvements on the MVTec AD dataset over prior methods. Remarkably, ONER achieves this with only 0.019M parameters and 5 training epochs per task, confirming its efficiency and stability for real-world industrial deployment.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/3_0_Formulation.tex <==
\section{Preliminaries}
\subsection{Problem Formulation}
%In  our incremental anomaly detection framework, the training and test sets are both partitioned into $N$ subsets according to the image categories. Specifically, $N$ is equal to 15 and 12 for the MVTec AD dataset and VisA dataset, respectively. The training set $\mathcal{T} = \{\mathcal{T}_1, \mathcal{T}_2, \ldots, \mathcal{T}_N\}$ consists exclusively of normal samples, while  the test set $\mathcal{T}^{\prime} = \{\mathcal{T}^{\prime}_1, \mathcal{T}^{\prime}_2, \ldots, \mathcal{T}^{\prime}_N\}$ is composed of both normal and anomalous samples.
In our incremental anomaly detection framework, the training and testing datasets are divided into $N$ distinct subsets, each corresponding to a distinct product category. The training set $\mathcal{T} = \{\mathcal{T}_1, \mathcal{T}_2, \ldots, \mathcal{T}_N\}$ contains normal samples only, whereas the test set $\mathcal{T}^{\prime} = \{\mathcal{T}^{\prime}_1, \mathcal{T}^{\prime}_2, \ldots, \mathcal{T}^{\prime}_N\}$ includes mixed normal and anomalous samples.

% The training set, denoted as $\mathcal{T} = \{\mathcal{T}_1, \mathcal{T}_2, \ldots, \mathcal{T}_N\}$, is made up exclusively of normal samples. In contrast, the test set, represented as $\mathcal{T}^{\prime} = \{\mathcal{T}^{\prime}_1, \mathcal{T}^{\prime}_2, \ldots, \mathcal{T}^{\prime}_N\}$, includes a mixture of normal and anomalous samples.

The model undergoes $N$ sequential training steps, incrementally learning from each subset $\mathcal{T}_t$, $t \in [1, N]$. Unlike frameworks that employ sample replay, our model operates in a strict rehearsal-free manner, prohibited from revisiting training data from previous steps~(i.e. steps 1 to $t -1$). After full incremental training, the final model is evaluated on the entire test set $\mathcal{T}^{\prime}$, performing anomaly detection without product identity priors.

% The general training process is divided into $N$ steps and the model is sequentially trained in each subset $\mathcal{T}_t$, $t \in [1, N]$. In contrast to frameworks that employ sample replay, our model is constrained from re-accessing training data from previous steps (i.e. steps 1 to $t -1$). After training, the final trained model is subjected to evaluation against the entire test set $\mathcal{T}^{\prime}$, without knowing the identity of the input product. 
% This scenario encapsulates a significant challenge, as there is a propensity for the model to experience catastrophic forgetting throughout the training process.

\subsection{Experience Formation}
In incremental learning, effectively leveraging experience from previous tasks is critical to mitigate catastrophic forgetting~\cite{rolnick2019experience}. This forgetting primarily stems from two factors: knowledge overwriting during parameter updates and feature conflicts between tasks. To address these issues, our framework incorporates two key experience components~(shown in Fig. \ref{fig:framework}): decomposed prompts and semantic prototypes, which jointly optimize model parameters and feature representations through its corresponding memory bank.

\subsubsection{Decomposed Prompts}
To retain historical knowledge while adapting to new tasks, we introduce decomposed prompts $\mathcal{D}=\{\mathbf{d}_{1}, \mathbf{d}_{2}, \ldots, \mathbf{d}_\text{N}\}$, which enable knowledge reuse from previous tasks while expanding learnable parameters for new tasks, with historical parameters frozen to prevent overwriting. 

Inspired by \cite{smith2023coda},  $\mathcal{D}$ consists of three key components: attention queries $\mathbf{q} \in \mathbb{R}^{M \times d}$, keys $\mathbf{k}\in \mathbb{R}^{M \times d}$ and prompt values $\mathbf{v}\in \mathbb{R}^{M\times L_p \times d}$, where $d$ is the embedding dimension, $L_p$ the prompt length, and $M=M_c\times N$ the total number of prompt components. Each $\mathbf{d}_\text{i}$ is thus represented as a tuple $\{\mathbf{q}_\text{i},\mathbf{k}_\text{i},\mathbf{v}_\text{i}\}$. 

When a new task $t$ arrives, the prompt bank expands by adding $M_c$ learnable components $\mathbf{d}_{\text{t}^*}=\{\mathbf{a}_{\text{t}^*},\mathbf{k}_{\text{t}^*},\mathbf{e}_{\text{t}^*}\}$, while freezing all previous components $\mathcal{D}_{t-1}=\{\mathbf{d}_{1}, \mathbf{d}_{2},\ldots, \mathbf{d}_\text{{t-1}}\}$. The expanded prompt bank is represented as $\mathcal{D}_{t^*}=\{\mathbf{d}_{1}, \mathbf{d}_{2},\ldots,\mathbf{d}_{\text{t}-1}, \mathbf{d}_{\text{t}^*}\}$, with only $\mathbf{d}_{\text{t}^*}$ is optimized during task $t$.

For each input image $x$, a corresponding prompt $p$ is generated via attention-weighted aggregation of prompt values: 
\begin{equation}
    p=\alpha \mathbf{v},
\end{equation}

where $\alpha$ is computed as the cosine similarity between the image feature query $q(x)$ and keys $\mathbf{k}$:
\begin{equation}
     \alpha = \gamma(q(x),\mathbf{k}), q(x) = f_\theta(x)\odot \mathbf{q}.
\end{equation}

Here, $f_\theta(x)$ denotes features extracted by a pre-trained ViT backbone.

Once the prompt $p$ is created, it is inserted into layers of $f_\theta$, forming an adapted model $f_\phi(x)=f_{\theta, \mathcal{D}}(x)$.
% $\gamma$ denotes the cosine similarity between the query $q(x) = f_\theta(x) \odot A$ and the keys $\mathbf{k}$, where $f_\theta(x) \in \mathbb{R}^D$ is the feature vector extracted from the pre-trained ViT $f_\theta$, and the operator $\odot$ represents element-wise product.

% Once the prompt $p$ is created, it is inserted into layers of $f_\theta$, resulting in a modified model $f_\phi(x)=f_{\theta, \mathcal{D}}(x)$. During both training and inference, we use $f_\phi$ to extract features from the input images, leveraging the enhanced representation provided by the inserted prompt.

\subsubsection{Semantic Prototypes}
% Semantic prototypes enforce regularization by explicitly enlarging feature distances between past and current tasks, thereby enhancing inter/intra-task discriminability and mitigating feature conflicts. To achieve this, they comprise \textbf{image-level} and \textbf{pixel-level} prototypes, which capture global and local representative features, respectively.
The semantic prototype bank stores two complementary representations: image-level prototypes for global semantic consistency and pixel-level prototypes for local discriminability, thus minimizing feature conflicts~\cite{tang2024incremental} and mitigating catastrophic forgetting.

The image-level prototypes $\mathcal{I}=\{\mathbf{i}_1, \mathbf{i}_2,\ldots, \mathbf{i}_\text{N}\}$ store a set of high-level feature center $\mathbf{i}_\text{i}\in\mathbb{R}^{1 \times d}$. During training, these prototypes enforce inter-task separation by regularizing feature distances.

The pixel-level prototypes $\mathcal{P}=\{\mathbf{p}_1, \mathbf{p}_2,\ldots, \mathbf{p}_\text{N}\}$ capture finer, task-specific details. Each  $\mathbf{p}_\text{i}\in\mathbb{R}^{N_s \times d}$ captures fine-grained normal patterns from $N_s$ representative patches per task. These prototypes mitigate feature conflicts by preserving local discriminability across tasks.
% consists of representative pixel-level features $\mathbf{p}_\text{{i, j}}\in\mathbb{R}^{1 \times d}$ for $j\in[1,N_s]$, where $N_s$ is the number of features selected for each task.  These prototypes mitigate feature conflicts by preserving local discriminability across tasks.

When processing task $t$, we retrieve the learned semantic prototypes $\mathcal{I}_{t-1}=\{\mathbf{i}_1, \mathbf{i}_2,\ldots, \mathbf{i}_\text{{t-1}}\}$ and $\mathcal{P}_{t-1}=\{\mathbf{p}_1, \mathbf{p}_2,\ldots, \mathbf{p}_\text{{t-1}}\}$ to perform regularization in the latent space. New prototypes $\mathbf{i}_\text{t}$ and $\mathbf{p}_\text{t}$ are selected from task $t$, incrementally added to the bank, and frozen, ensuring stable long-term knowledge retention.

% The previous semantic prototypes $\mathcal{I}_{t-1}$ and $\mathcal{P}_{t-1}$ are used to optimize the current task's Decomposed Prompts $\mathcal{D}_{t^*}$, as well as to select current semantic prototypes $\mathbf{i}_\text{t}$ and $\mathbf{p}_\text{t}$.  Once selected, prototypes $\mathbf{i}_\text{t}$ and $\mathbf{p}_\text{t}$ are stored in memory and frozen to prevent further modification.

==> sections/3_Method.tex <==
\section{Methods}

\subsection{Overview}
The training process is divided into $N$ sequential steps, each corresponding to a distinct task category. At each step $t \in [1, N]$, the model adapts to the current task $\mathcal{T}_t$ while preserving knowledge from previous tasks. Detailed algorithmic training procedure are provided in the Appendix.

Specifically, at the pre-stage of task $t$, the previous Decomposed Prompts $\mathcal{D}_{t-1}$ are expanded to $\mathcal{D}_{t^*}$. Concurrently, historical Image-level Prototypes $\mathcal{I}_{t-1}$ are retrieved and fed into the \textbf{ Incremental Refinement of Image-level Prototypes (IRIP) } module alongside the current training data $\mathcal{T}_t$. IRIP generates a refined image-level prototype $\mathbf{i}_\text{t}$ for the current task, updating the prototype bank as: 
\begin{equation}
    \mathcal{I}_{t}=\mathcal{I}_{t-1} \cup \mathbf{i}_\text{t}.
\end{equation}

During task training, each image $x \in \mathcal{T}_t$ is processed through the model $f_\phi$ to extract normalized features $\mathbf{k}$, which are partitioned into an image-level feature $\mathbf{k}_\text{I}\in\mathbb{R}^{1 \times d}$ and pixel-level features $\mathbf{k}_\text{P}\in \mathbb{R}^{N_p \times d}$, where $N_p$ is the number of patches. These features, along with $\mathcal{I}_{t}$ and retrieved $\mathcal{P}_{t-1}$, are then processed by the \textbf{ Experience Replay-based Optimization (ERO) } module to compute $\mathcal{L}_{\text{align}}$, $\mathcal{L}_{\text{TSC}}$ and $  \mathcal{L}_{\text{ITC}}$. The total loss $\mathcal{L}_\text{total}=\mathcal{L}_{\text{align}}+\mathcal{L}_{\text{TSC}}+\mathcal{L}_{\text{ITC}}$ optimizes $\mathcal{D}_{t^*}$, producing the updated prompts $\mathcal{D}_{t}$.

Once the training of task $t$ is complete, the \textbf{Incremental Selection of  Pixel-level Prototypes(ISPP)} module selects representative prototypes $\mathbf{p}_\text{t}$ from $ \mathcal{T}_t$, utilizing $\mathcal{D}_{t}$ and $\mathcal{P}_{t-1}$. These prototypes are merged into the global bank:
\begin{equation}
    \mathcal{P}_{t} = \mathcal{P}_{t-1}  \cup \mathbf{p}_\text{t}.
\end{equation}

% This process ensures incremental refinement of knowledge across tasks, effectively preserving past knowledge while optimizing the model’s performance on new tasks and mitigating catastrophic forgetting.
\begin{table*}[!ht]
    \centering
    {\small
    \begin{tabular}{lccccccccc}
    \toprule
    \multirow{2}{*}{Method}& Extra info& 
    \multicolumn{2}{c}{Image-level ACC~$\uparrow$} & \multicolumn{2}{c}{Image-level FM~$\downarrow$}& 
    \multicolumn{2}{c}{Pixel-level ACC~$\uparrow$} & \multicolumn{2}{c}{Pixel-level FM~$\downarrow$}\\
       \cmidrule(lr){2-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6}  \cmidrule(lr){7-8} \cmidrule(lr){9-10}
        ~&SR~$|$~TI~$|$~ED&AUROC & AUPR & AUROC & AUPR &AUROC & AUPR &  AUROC & AUPR\\
   % ~ &~&~&~&AUROC & AP & F1 Max & AUROC & AP & F1 Max  \\ 
   \midrule
   % \multicolumn{14}{l}{\textit{Training-based AD}\\
   \textit{Training-based ADs:}\\
        \hspace{1em}DRAEM~\textcolor{gray}{\tiny [ICCV21]} & $\times|\times|\times$&57.7&78.7&39.4&20.0&61.6&11.7&34.3&53.6\\
        % \hspace{1em}GLAD \textcolor{gray}{\tiny [ECCV24]}&$\times|\times|\times$&76.1&88.5&87.1&21.3&10.3&10.2&88.7&32.6&35.9&9.5&32.7&28.6\\
        \hspace{1em}BGAD~\textcolor{gray}{\tiny [CVPR23]} & $\times|\times|\times$ &51.8&73.9&42.1&22.6&50.5&6.6&46.0&48.0 \\
        % \hspace{1em}SimpleNet \textcolor{gray}{\tiny [CVPR23]}&$\times|\times|\times$&57.5&78.5&84.1&41.9&21.3&14.6&52.0&5.7&10.3&45.6&48.8&46.4\\
        \hspace{1em}DRAEM-Replay &$\checkmark|\times|\times$&74.9&87.7&22.3&11.1&85.0&\underline{37.6}&10.8&27.7\\
        \hspace{1em}BGAD-Replay &$\checkmark|\times|\times$&79.9&89.5&14.0&7.0&\underline{91.3}&33.0&5.1&21.7\\
        \hspace{1em}DRAEM-CLS* &$\checkmark|\times|\times$&80.6&87.1&16.5&11.7&82.7&29.7&13.2&35.6\\
        \hspace{1em}BGAD-CLS* &$\checkmark|\times|\times$&83.4&89.3&10.5&7.2&84.8&24.5&11.7&30.1\\
        % \midrule
        \hline
   \textit{Training-free ADs:}\\
        \hspace{1em}WinCLIP \textcolor{gray}{\tiny [CVPR23]}&$\times|\checkmark|\times$&90.4&95.6&/&/&82.3&18.2&/&/\\
        \hspace{1em}SAA++ \textcolor{gray}{\tiny [Arxiv23]}&$\times|\checkmark|\times$&63.1&81.4&/&/&73.2&28.8&/&/\\
        \hspace{1em}CLIP-Surgery~\textcolor{gray}{\tiny [Arxiv23]} &$\times|\checkmark|\times$&90.2&95.5&/&/&83.5&23.2&/&/\\

        \hspace{1em}FADE~\textcolor{gray}{\tiny [BMVC24]} & $\times|\checkmark|\times$& 90.1&95.5&/&/&89.2&39.8&/&/\\
        \hspace{1em}SDP~\textcolor{gray}{\tiny [Arxiv24]} &$\times|\checkmark|\times$&90.9&95.8&/&/&87.5&30.4&/&/\\
        \hspace{1em}AnomalyCLIP~\textcolor{gray}{\tiny [ICLR24]} &$\times|\checkmark|\checkmark$&91.6&96.4&/&/&91.1&34.5&/&/\\
        \hspace{1em}SDP+~\textcolor{gray}{\tiny [Arxiv24]} &$\times|\checkmark|\checkmark$&\underline{92.2}&\underline{96.6}&/&/&91.2&36.3&/&/\\
        \hspace{1em}PatchCore*~\textcolor{gray}{\tiny [CVPR22]} &$\times|\times|\times$&90.4&94.9&\underline{0.7}&\underline{0.3}&89.7&22.1&\underline{3.8}&19.3\\
        % \midrule
        \hline
       \textit{Incremental ADs:}\\

        \hspace{1em}CAD~\textcolor{gray}{\tiny [ACM MM23]}&$\times|\times|\times$&87.1&93.3&1.9&1.7&/&/&/&/\\
        \hspace{1em}CAD~+~PANDA&$\times|\times|\times$&47.8&74.1&36.0&18.5&/&/&/&/\\
       \hspace{1em}CAD~+~CutPaste & $\times|\times|\times$&74.6&86.3&17.2&10.0&/&/&/&/ \\
        \hspace{1em}IUF~\textcolor{gray}{\tiny [ECCV24]} &$\times|\times|\times$&71.3&83.9&3.9&1.1&79.0&16.0&5.7&\underline{6.7}\\
        \hspace{1em}UCAD*~\textcolor{gray}{\tiny [AAAI24]} &$\times|\times|\times$&90.7&95.3&1.8&0.9&90.1&21.4&6.1&24.2\\
        % \midrule
        % \cmidrule(lr){3-14}
        \hspace{1em}\textbf{Ours} &$\times|\times|\times$&\textbf{93.4}&\textbf{97.3}&\textbf{0.6}&\textbf{0.1}&\textbf{94.5}&\textbf{49.7}&\textbf{0.9}&\textbf{1.3}\\
        \bottomrule
    \end{tabular}}
    \caption{{Comparison of Pixel-level and Image-level ACC and FM on the MVTec AD dataset ($N=15$) after training on the last subdataset. Note that * signifies staged approaches. Bold and underline highlight the best and second-best results.}}
    \label{tab:mvtec-sota}
\end{table*}
\begin{table*}[!ht]
    \centering
    {\small
    \begin{tabular}{lccccccccc}
    \toprule
    \multirow{2}{*}{Method}& Extra info& 
    \multicolumn{2}{c}{Image-level ACC~$\uparrow$} & \multicolumn{2}{c}{Image-level FM~$\downarrow$}& 
    \multicolumn{2}{c}{Pixel-level ACC~$\uparrow$} & \multicolumn{2}{c}{Pixel-level FM~$\downarrow$}\\
       \cmidrule(lr){2-2} \cmidrule(lr){3-4} \cmidrule(lr){5-6}  \cmidrule(lr){7-8} \cmidrule(lr){9-10}
        ~&SR~$|$~TI~$|$~ED&AUROC & AUPR & AUROC & AUPR &AUROC & AUPR &  AUROC & AUPR\\
   % ~ &~&~&~&AUROC & AP & F1 Max & AUROC & AP & F1 Max  \\ 
   \midrule
   \textit{Training-based ADs:}\\
        \hspace{1em}DRAEM~\textcolor{gray}{\tiny [ICCV21]} & $\times|\times|\times$&50.2&60.0&44.2&35.5&60.5&5.0&33.3&28.5 \\
        % \hspace{1em}GLAD \textcolor{gray}{\tiny [ECCV24]}&$\times|\times|\times$&76.8&78.7&80.3&3.0&3.0&3.6&88.6&11.8&18.1&4.9&3.9&\textbf{1.5}\\
        \hspace{1em}BGAD~\textcolor{gray}{\tiny [CVPR23]} & $\times|\times|\times$ & 52.0&59.9&42.0&34.7&58.9&5.8&39.8&34.9\\
        % \hspace{1em}SimpleNet \textcolor{gray}{\tiny [CVPR23]}&$\times|\times|\times$&50.3&57.8&44.5&38.3&57.0&1.6&39.1&32.5\\
        \hspace{1em}DRAEM-Replay &$\checkmark|\times|\times$&81.4&84.8&13.0&10.7&81.9&16.4&11.8&17.2\\
        \hspace{1em}BGAD-Replay &$\checkmark|\times|\times$&80.0&82.6&14.0&12.0&95.2&22.1&3.4&18.6\\
        \hspace{1em}DRAEM-CLS* &$\checkmark|\times|\times$&\underline{83.3}&85.4&11.0&10.1&83.9&17.4&9.9&16.2\\
        \hspace{1em}BGAD-CLS* &$\checkmark|\times|\times$&\textbf{84.6}&\underline{85.5}&9.4&9.1&89.7&\underline{20.8}&9.0&19.9\\
        % \midrule
        \hline
        \textit{Training-free ADs:}\\
        \hspace{1em}WinCLIP \textcolor{gray}{\tiny [CVPR23]}&$\times|\checkmark|\times$&75.5&78.7&/&/&73.2&5.4&/&/\\
        \hspace{1em}SAA++ \textcolor{gray}{\tiny [Arxiv23]}&$\times|\checkmark|\times$&71.1&77.3&/&/&74.0&22.4&/&/\\
        \hspace{1em}CLIP-Surgery~\textcolor{gray}{\tiny [Arxiv23]} &$\times|\checkmark|\times$&76.8&80.2&/&/&85.0&10.3&/&/\\

        \hspace{1em}FADE~\textcolor{gray}{\tiny [BMVC24]} & $\times|\checkmark|\times$&74.7&78.5&/&/&91.0&10.0&/&/ \\
        \hspace{1em}SDP~\textcolor{gray}{\tiny [Arxiv24]} &$\times|\checkmark|\times$&78.6&81.5&/&/&88.1&12.2&/&/\\
        \hspace{1em}AnomalyCLIP~\textcolor{gray}{\tiny [ICLR24]} &$\times|\checkmark|\checkmark$&82.0&85.3&/&/&\textbf{95.5}&21.3&/&/\\
        \hspace{1em}SDP+~\textcolor{gray}{\tiny [Arxiv24]} &$\times|\checkmark|\checkmark$&78.3&79.0&/&/&\underline{94.0}&18.1&/&/\\
        \hspace{1em}PatchCore*~\textcolor{gray}{\tiny [CVPR22]} &$\times|\times|\times$&78.7&82.7&\textbf{1.0}&\textbf{0.8}&88.7&15.9&\textbf{2.2}&9.1\\
        % \midrule
        \hline
        \textit{Incremental ADs:}\\
        \hspace{1em}CAD~\textcolor{gray}{\tiny [ACM MM23]}&$\times|\times|\times$&64.7&70.7&13.8&11.3&/&/&/&/\\
        \hspace{1em}CAD~+~PANDA&$\times|\times|\times$&55.6&65.9&19.3&12.8&/&/&/&/\\
        \hspace{1em}CAD~+~CutPaste & $\times|\times|\times$& 65.9&71.0&13.5&11.2&/&/&/&/\\
        \hspace{1em}IUF~\textcolor{gray}{\tiny [ECCV24]} &$\times|\times|\times$&65.9&85.2&\underline{2.6}&4.7&85.6&3.8&\underline{2.3}&\textbf{1.6}\\
        \hspace{1em}UCAD*~\textcolor{gray}{\tiny [AAAI24]} &$\times|\times|\times$&75.7&79.2&10.8&8.9&86.9&10.1&5.9&19.8\\
        % \midrule
        % \cmidrule(lr){3-14}
        \hspace{1em}\textbf{Ours} &$\times|\times|\times$&83.1&\textbf{86.6}&3.9&\underline{2.7}&90.6&\textbf{27.9}&2.4&\underline{1.8}\\
        \bottomrule
    \end{tabular}}
    \caption{{Comparison of Pixel-level and Image-level ACC and FM on the VisA dataset ($N=12$) after training on the last subdataset. Note that * signifies staged approaches. Bold and underline highlight the best and second-best results.}}
    \label{tab:visa-sota}
\end{table*}

\begin{table}[t]
\centering
\small
% {\footnotesize
\begin{tabular}{lcc}
\toprule
Method & Learnable Parameters & Epochs \\
\midrule
DRAEM~\textcolor{gray}{\tiny [ICCV21]} & 97.42M & 300 \\
% GLAD~\textcolor{gray}{\tiny [ECCV24]} & 859.52M  & 280\\
BGAD~\textcolor{gray}{\tiny [CVPR23]} & 3.39M & 100 \\
% STPM~\textcolor{gray}{\tiny [BMVC21]} & & \\
% SimpleNet~\textcolor{gray}{\tiny [CVPR23]} & 3.94M & 160 \\
% \midrule
DRAEM-Replay & 97.42M & 300\\
BGAD-Replay & 3.39M & 100\\
DRAEM-CLS* & (97.42+8.40)M & 300+10\\
BGAD-CLS* & (3.39+8.40)M & 100+10\\
% \midrule
\hline


CAD~\textcolor{gray}{\tiny [ACM MM23]} & 85.21M & 50 \\
IUF~\textcolor{gray}{\tiny [ECCV24]} & 9.11M & 200 \\
UCAD*~\textcolor{gray}{\tiny [AAAI24]} & 0.021M & 25 \\

% \midrule
\hline
\textbf{ONER} (Ours) & \textbf{0.019M} & \textbf{5} \\
\bottomrule
\end{tabular}
\caption{Statistics of learnable parameters and training epochs per task for different methods.}
\label{tab:parameter_epochs_statistics}

\end{table}
\subsection{Incremental Refinement of Image-level Prototypes}
The incremental refinement of image-level prototypes establishes implicit semantic boundaries across tasks by dynamically aligning task-specific representations while preserving historical knowledge. 

At step $t$, previously stored prototypes $\mathcal{I}_{t-1}$ serve as reference anchors to guide the refinement of the current task’s prototype. The initial prototype $\mathbf{i}_\text{init}$ is derived as the mean image-level feature of the current task’s data using the pretrained model $f_\theta$. To optimize $\mathbf{i}_\text{t}$, we propose the Image-level Prototype Refinement Loss $\mathcal{L}_{\text{IPR}}$, which balances two objectives:

\begin{itemize}
    \item Similarity Preservation Loss $\mathcal{L}_{\text{sim}}$ maximizes the cosine similarity between the refined prototype $\mathbf{i}_\text{t}$ and the initial prototype $\mathbf{i}_\text{init}$:

    \begin{equation}
        \mathcal{L}_{\text{sim}} = -\cos \left( \mathbf{i}_\text{t}, \mathbf{i}_\text{init} \right).
    \end{equation}
    \item Inter-Task Distinction Loss $\mathcal{L}_{\text{dist}}$ minimizes the maximum cosine similarity between $\mathbf{i}_\text{t}$ and the prototypes stored in  $\mathcal{I}_{t-1}$:
    \begin{equation}
        \mathcal{L}_{\text{dist}} = \max_{\mathbf{i} \in \mathcal{I}_{t-1}} \cos \left( \mathbf{i}_\text{t}, \mathbf{i} \right).
    \end{equation}
\end{itemize}
The total refinement loss $\mathcal{L}_{\text{IPR}}=\mathcal{L}_{\text{sim}} +   \mathcal{L}_{\text{dist}}$ is minimized using the LBFGS optimizer,  yielding the refined prototype to minimize $\mathcal{L}_{\text{IPR}}$, and then update the prototypes $\mathbf{i}_\text{t}$, which is then added to the prototype bank $\mathcal{I}_{t}=\mathcal{I}_{t-1} \cup \mathbf{i}_\text{t}$. This dual-objective optimization ensures that prototypes simultaneously capture task-specific semantics and avoid interference with historical knowledge. Detailed algorithmic steps are provided in the Appendix.


\subsection{Experience Replay-based Optimization}
In experience replay-based optimization, we leverage previous experience to refine the model, incorporating both inter-task and intra-task optimization. Inter-task optimization enhances feature discriminability across tasks to mitigate feature conflicts, while intra-task optimization strengthens task-specific representations for pixel-level retrieval during inference.
\subsubsection{Inter-task optimization}
To enhance inter-task feature discriminability, thus mitigating feature conflict across tasks, the Image-Level Prototype Alignment Loss $\mathcal{L}_\text{align}$ and the Inter-Task Contrastive Loss $ \mathcal{L}_{\text{ITC}}$ are applied: 

 \begin{equation}
     \begin{aligned}
     &\mathcal{L}_{\text{align}} = \left\| \mathbf{k}_\text{I} - \mathbf{i}_\text{t}\right\|_2,\\
     &\mathcal{L}_{\text{ITC}} = \sum_{i\in N_p} \max_{\mathbf{p} \in \mathcal{P}_{t-1}} \cos \left(\mathbf{k}_\text{{P,i}}, \mathbf{p}\right),
     \end{aligned}
 \end{equation}
where $\mathcal{L}_\text{align}$ minimizes the L2 divergence between the current image-level feature $\mathbf{k}_\text{I}$ and the refined prototype $\mathbf{i}_\text{t}\in \mathcal{I}_{t}$, and $ \mathcal{L}_{\text{ITC}}$ reduces similarity between the current patch features and those stored in $\mathcal{P}_{t-1}$.

This dual-loss strategy explicitly separates task-specific features, preventing semantic overlap.
\subsubsection{Intra-task optimization}
To enhance task-specific representation, the Task-Specific Contrastive Loss $\mathcal{L}_{\text{TSC}}$  integrates class-aware constraints. Leveraging SAM~\cite{kirillov2023segment} for segmentation, we assign class labels $C_{{P, i}}$ to patch features $\mathbf{k}_{\text{P,i}}$. The loss comprises:

% Specifically, following UCAD's framework, we use pre-trained models such as SAM \cite{kirillov2023segment} for segmentation. Each patch feature $\mathbf{k}_{\text{P,i}}$ is assigned to its corresponding class labels $C_{{P, i}}$.

% For each input image $x$, we extract its pixel-level features $\mathbf{k}_\text{p}=f_{\phi}(x)$. $\mathcal{L}_{\text{TSC}}$ consists of two components: $ \mathcal{L}_{\text{pos}}$, measuring intra-class similarity, and $\mathcal{L}_{\text{neg}}$, measuring inter-class dissimilarity. These loss functions are defined as follows:
\begin{equation}
    \begin{aligned}
    &\mathcal{L}_{\text{pos}} = \sum_{i,j \in {N}_p} \cos \left (\mathbf{k}_\text{{P,i}}, \mathbf{k}_\text{{P, j}} \right), C_{{P, i}}=C_{P, j}, \\
    &\mathcal{L}_{\text{neg}} = \sum_{i,j \in {N}_p} \cos \left (\mathbf{k}_\text{{P, i}}, \mathbf{k}_\text{{P, j}} \right ), C_{{P, i}}\neq C_{{P, j}}, \\
    &\mathcal{L}_{\text{TSC}} = \mathcal{L}_{\text{pos}} - \mathcal{L}_{\text{neg}}.\\
    \end{aligned}
\end{equation}
By maximizing intra-class similarity ($\mathcal{L}_{\text{pos}}$) and minimizing inter-class similarity~($\mathcal{L}_{\text{neg}}$), the model learns compact and discriminative representations for precise anomaly localization.
\subsection{Incremental Selection of  Pixel-level Prototypes}
This module ensures memory-efficient and conflict-aware prototype retention by incrementally selecting pixel-level features that balance intra-task representativeness and inter-task discriminability. Unlike prior methods~\cite{Roth_2022_CVPR, liu2024unsupervised} that prioritize task-specific feature selection at the cost of cross-task interference, our approach explicitly enforces implicit semantic boundaries across tasks, mitigating feature conflicts while preserving critical anomaly patterns.

After training task $t$, the pretrained model $f_\phi$ extracts pixel-level features from $\mathcal{T}_t$, forming a feature matrix $\mathbf{p}_\text{all} \in \mathbb{R}^{N_I \times N_p \times d}$, where $N_I$ is the number of samples in $\mathcal{T}_t$, and $N_p$ is the number of patches per image.

To optimize storage and inference efficiency, we select $N_s=N_p$ pixel-level features $\mathbf{p}_\text{t} \in \mathbf{p}_\text{all}$ that maximize representativeness while minimizing redundancy.

Existing methods rely on greedy algorithms to select task-specific features but ignore inter-task differentiation, risking semantic overlap. In contrast, our selection process jointly optimizes intra-task coverage and inter-task separation through a two-step strategy: 

\begin{enumerate}
    \item Coreset Selection: Prototypes are selected by minimizing the maximum distance between any feature in $\mathbf{p}_\text{all}$ and the nearest prototype in either the current coreset $\mathcal{E}_C$ or historical prototypes $\mathcal{P}_{t-1}$:
    % \item Select $\mathbf{p}_\text{t}$ from $\mathbf{p}_\text{all}$ by minimizing the maximum distance between any feature in $\mathbf{p}_\text{all}$ and the nearest feature in the coreset $\mathcal{E}_C$ or the previously stored prototypes $\mathcal{P}_{t-1}$:
    \begin{equation}
        \mathbf{p}_\text{t} = \arg\min_{\mathcal{E}_C \subseteq \mathbf{p}_\text{all}}  \max_{m \in \mathbf{p}_\text{all}} \min_{n \in \mathcal{E}_C\cup\mathcal{P}_{t-1}} \| m - n \|^2.
    \end{equation}
 
    \item Prototype Integration: The selected prototypes are merged into the global prototype bank:
   \begin{equation}
    \mathcal{P}_{t} = \mathcal{P}_{t-1}  \cup \mathbf{p}_\text{t}.
\end{equation}
\end{enumerate}
By enforcing both intra-task representativeness and inter-task separation, the prototype bank $\mathcal{P}$ retains task-specific semantics while preventing cross-task contamination, thereby enhancing incremental anomaly detection robustness.





==> sections/supplementation.tex <==
\clearpage

\setcounter{page}{1}
\maketitlesupplementary
\begin{appendices}
\renewcommand{\thesection}{\Alph{section}}
% \section{Training and inference procedure}
% The training process is divided into $N$ steps, with each step corresponding to a specific task category. During each step $t \in [1, N]$, the model is sequentially trained on the subset $\mathcal{T}_t$. The training procedure is designed to ensure that the model effectively incorporates new knowledge from the current task while preserving previously acquired knowledge, as described in Algo.~\ref{alg:train}. To provide further clarity, we present a comprehensive description of the \textbf{IRIP} module. The corresponding procedure of refining image-level prototype is outlined in Algo.~\ref{alg:ICGOM}.
% \begin{algorithm}[tp]
% \caption{Training}
% \label{alg:train}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \definecolor{codeblue}{rgb}{0.25,0.5,0.5}
% \textcolor{codeblue}{\# The overall training process is divided into N steps, for each step $t\in [1, N]$:}
% \begin{algorithmic}[1]
% \REQUIRE{
%     Pretrained ViT $f_\theta$,
%     Training datasets $\mathcal{T}_t \in \{\mathcal{T}_1, \mathcal{T}_2, \ldots, \mathcal{T}_N\}$, 
%     $\mathcal{D}_{t-1}$,
%     $\mathcal{I}_{t-1}$,
%     $\mathcal{P}_{t-1}$
% }\\
% \ENSURE{
%     $\mathcal{D}_{t}$,
%     $\mathcal{I}_{t}$,
%     $\mathcal{P}_{t}$
% }\\
% % \FOR{$t:= 1~\text{to}~N$}
%     \STATE \textcolor{codeblue}{\# Pre-stage:}
%     \STATE  \textbf{expand} $\mathcal{D}_{t^*}\gets \mathcal{D}_{t-1} \cup  \mathbf{d}_{\text{t}^*}$
%     % \STATE \textcolor{codeblue}{\# 2.update Image-level Prototypes}
%     \STATE $\mathbf{i}_\text{t} \gets \textbf{IRIP}( \mathcal{I}_{t-1}, \mathcal{T}_t)$ \textcolor{codeblue}{\# refers to section 4.2}
%     \STATE \textbf{update} $\mathcal{I}_{t} \gets \mathcal{I}_{t-1} \cup \mathbf{i}_\text{t}$
%     \STATE \textcolor{codeblue}{\# Training stage:}
%     \WHILE{training not converged}
%      \FOR{batch $x \in \mathcal{T}_t$}
%     \STATE $\mathbf{k}_\text{I},\mathbf{k}_\text{P} \gets f_{\theta, \mathcal{D}_{t^*}}(x)$
%     % \STATE \textcolor{codeblue}{\# 2.loss computation}
%     \STATE $\mathcal{L}_\text{align},\mathcal{L}_\text{TSC},\mathcal{L}_\text{ITC} \gets \textbf{ERO}(\mathcal{I}_{t},\mathbf{k}_\text{I},\mathcal{P}_{t-1},\mathbf{k}_\text{P})$ \textcolor{codeblue}{\# refers to section 4.3}
%     \STATE $\mathcal{L}_\text{total} =\mathcal{L}_\text{align} + \mathcal{L}_\text{TSC} + \mathcal{L}_\text{ITC}$
%     % \STATE \textcolor{codeblue}{\# 3.backward propagation}
%     \STATE $ \mathcal{D}_{t^*} \gets \textbf{BP}(\mathcal{L}_\text{total})$
%     \ENDFOR
%     \ENDWHILE
   
%     \STATE \textcolor{codeblue}{\# Post-stage:}
%     \STATE \textbf{fix} $\mathcal{D}_{t} \gets \mathcal{D}_{t^*}$
%     % \STATE \textcolor{codeblue}{\# 2.update Pixel-level Prototypes}
%     \STATE $\mathbf{p}_\text{t} \gets \textbf{ISPP}(\mathcal{T}_t,\mathcal{D}_{t},\mathcal{P}_{t-1})$ \textcolor{codeblue}{\# refers to section 4.4}
%     \STATE \textbf{update} $\mathcal{P}_{t} \gets \mathcal{P}_{t-1} \cup \mathbf{p}_\text{t}$
% % \ENDFOR
% \STATE \textbf{Return:}  $\mathcal{D}_{t}$,
%     $\mathcal{I}_{t}$,
%     $\mathcal{P}_{t}$
% \end{algorithmic}
% \end{algorithm}
% \begin{algorithm}[tp]
% \caption{IRIP}
% \label{alg:ICGOM}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \definecolor{codeblue}{rgb}{0.25,0.5,0.5}
% % \textcolor{codeblue}{\# Incremental Refinement of Image-level Prototypes during task t}
% \begin{algorithmic}[1]
% \REQUIRE{
%     $\mathcal{I}_{t-1}, \mathcal{T}_t$
% }\\
% \ENSURE{
%     $\mathbf{i}_\text{t}$
% }\\
% \STATE \textcolor{codeblue}{\# 1.calculate the average of features extracted by $f_\theta$ in dataset $\mathcal{T}_t$}
% \STATE $I_\text{init} = \overline{f_\theta(x)}$ for $x \in \mathcal{T}_t$

% \STATE $\mathbf{i}_\text{t}=I_\text{init}$
% \IF{$t>1$}
% \STATE \textcolor{codeblue}{\# 2.update $\mathbf{i}_\text{t}$ using LBFGS optimizer}
%     \FOR{$e = 1$ \TO $nums_{epoch}$}
%         \STATE  $ \mathcal{L}_{\text{sim}} = -\cos \left( \mathbf{i}_\text{t}, I_\text{init} \right)$
%         \STATE $ \mathcal{L}_{\text{dist}} = \max_{\mathbf{i} \in \mathcal{I}_{t-1}} \cos \left( \mathbf{i}_\text{t}, \mathbf{i} \right)
% $
%         \STATE $\mathcal{L}_{\text{total}} =   \mathcal{L}_{\text{sim}} + \mathcal{L}_{\text{dist}}$
%         \STATE \textbf{update} $\mathbf{i}_{\text{t}} \gets$ optimizer\_{LBFGS}($\mathcal{L}_{\text{total}}$)
%     \ENDFOR
% \ENDIF
% \STATE \textbf{Return:} $\mathbf{i}_\text{t}$
% \end{algorithmic}
% \end{algorithm}

% After training, the fully trained model is evaluated on the complete test set $\mathcal{T}^{\prime}$. The anomaly score $s$ for each image $ x' \in \mathcal{T}^{\prime}$ is calculated. To be specific, we compare the image feature $m^{test} \in \mathbf{k}_\text{P}$
% with the pixel-level prototypes stored in $\mathcal{P}$. 
% Building upon patch-level retrieval, re-weighting is employed to enhance the anomaly detection process, as outlined in Algo.~\ref{alg:inference}. This approach refines the anomaly scores to improve detection accuracy.
% \begin{algorithm}
% \caption{Inference}
% \label{alg:inference}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}
% \definecolor{codeblue}{rgb}{0.25,0.5,0.5}
% % \textcolor{codeblue}{\# The inference process while dealing with images in task $t$:}
% \begin{algorithmic}[1]
% \REQUIRE{
%     Pretrained ViT $f_\theta$,
%     $ x' \in \mathcal{T}^{\prime}$,
%     $\mathcal{D}$,
%      $\mathcal{P}$ 
% }\\
% \ENSURE{
%     Anomaly Score $s$
% }\\
% \STATE \textcolor{codeblue}{\# 1.calculate the inserted prompt $p$}
% \STATE $\{\mathbf{q},\mathbf{k},\mathbf{v}\} \gets \mathcal{D}$
% \STATE $p \gets Sim(f_\theta(x') \odot\mathbf{q},\mathbf{k})\cdot\mathbf{v}$
% \STATE \textcolor{codeblue}{\# 2.calculate the pixel-level features}
% \STATE $\mathbf{k}_\text{P} \gets f_\phi(x') = f_{\theta,\mathcal{D}}(x')=f_{\theta,p}(x')$
% \STATE \textcolor{codeblue}{\# 3.calculate the anomaly score referred to \cite{roth2022towards}}
% % \STATE $s \gets \textbf{PatchCore}(k_p,\mathcal{E}_{\text{PIX}})$ \textcolor{codeblue}{\# Details of \textbf{PatchCore} referred to \cite{roth2022towards}}

% % \STATE \textcolor{codeblue}{\# Suppose $m^{test,*}$ is the feature in $k_p$, which keep the furthest distance between the  $\mathcal{E}_{\text{PIX}}$}
% \STATE $m^{test,*},m^{*}=\arg\max\limits_{m^{test} \in \mathbf{k}_\text{P}}\arg\min\limits_{m \in \mathcal{P}}\left\|m^{test}-m\right\|_2$
% \STATE  $s^{*}=\left\|m^{test,*}-m^{*}\right\|_2$ 
% % \STATE \textcolor{codeblue}{\# $\mathcal{N}_n(m^{*})$ represents the n-nearest neighbors of $m^{*}$ in $\mathcal{E}_{\text{PIX}}$;}
% \STATE  $s=(1-\frac{\exp{\left\|m^{test,*}-m^{*}\right\|_2}}{\sum_{m\in\mathcal{N}_n(m^{*})}\exp{\left\|m^{test,*}-m^{*}\right\|_2}}) \cdot s^{*}$ \textcolor{codeblue}{\# $\mathcal{N}_n(m^{*})$ represents the n-nearest neighbors of $m^{*}$ in $\mathcal{P}$;}
% \STATE \textbf{Return:} $s$
% \end{algorithmic} 
% \end{algorithm}



\begin{table*}[tp]
\centering
{\scriptsize
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\begin{tabular}{ccccccccccccccc}
\hline
\textbf{bottle} & \textbf{cable} & \textbf{capsule} & \textbf{carpet} & \textbf{grid} & \textbf{hazelnut} & \textbf{leather} & \textbf{metal\_nut} & \textbf{pill} & \textbf{screw} & \textbf{tile} & \textbf{toothbrush} & \textbf{transistor} & \textbf{wood} & \textbf{zipper} \\
\hline
91.57 & 98.67 & 100 & 90.60 & 75.64 & 79.09 & 50.81 & 99.13 & 98.20 & 100 & 94.02 & 80.95 & 100 & 88.61 &  91.39\\
\hline
\end{tabular}}
\caption{Classification accuracy for each category on the MVTec AD dataset at the task identification stage for UCAD.}
\label{tab:accuracy}
\end{table*}
\begin{table}[!ht]
\centering
{\footnotesize
\begin{tabular}{lcccc}
\toprule
\textbf{Method} & \multicolumn{2}{c}{\textbf{ACC} $\uparrow$} & \multicolumn{2}{c}{\textbf{FM} $\downarrow$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 &   \textbf{AUROC} & \textbf{AUPR} & \textbf{AUROC} & \textbf{AUPR} \\
\midrule
% \multicolumn{5}{l}{\textit{Incremental Anomaly Detection Methods}} \\
UCAD & 86.66 & 10.94 & 12.52 & 22.78 \\
Ours & \textbf{99.44} & \textbf{45.43} & \textbf{0.03} & \textbf{1.16}\\
\bottomrule
\end{tabular}}
\caption{Comparison of Pixel-level ACC and FM on the category leather of the MVTec AD dataset after training on the last subset.}
\label{tab:pixel-leather}
\end{table}
\section{Comparison with current sota method: UCAD~\cite{liu2024unsupervised}}
%UCAD utilizes contrastive prompt learning to introduce a continual prompting module that adapts to incremental tasks and facilitates segmentation. 
In the framework of UCAD, contrastive prompt learning is utilized to introduce a continual prompting module that adapts to incremental tasks and facilitates segmentation. 
%Besides, UCAD trains distinct prompts for each task and stores a triplet comprising the prompt, knowledge extracted using a ViT model, and key features stored in a memory bank. 
Besides, UCAD trains distinct prompt for each task and stores a triplet comprising the prompt, knowledge extracted by a ViT, and key features stored in a memory bank. 
%During inference, UCAD employs a two-stage process: it first identifies the task associated with the input image by comparing its features (extracted using a pre-trained ViT) with keys in the memory bank, then applies the corresponding prompt and knowledge to detect anomalies.
During inference, UCAD employs a two-stage process: it first identifies the task associated with the input image by comparing its features with keys in the memory bank, then applies the corresponding prompt and knowledge to detect anomalies.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/ucad-ex.png}
    \caption{Typical mismatch cases in UCAD. (a) An image from the leather category is mistakenly identified as wood. (b) An image from hazelnut category is mismatched as metal\_nut.}
    \label{fig:mismatch}
\end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{images/figure3-o.png}
    \caption{Impact of Task Misidentification on UCAD's Performance.}
    \label{fig:visual2}
\end{figure}
\begin{figure}[t]
\centering
\includegraphics[width=0.46\textwidth]{images/figure-cls.png} % Reduce the figure size so that it is slightly narrower than the column.
%\caption{Impact of Task Misidentification on Staged Model's Performance.}
\caption{Qualitative evaluation between stage approach and ours. Compared with stage approach which suffers from task misidentification (red), our method is more stable and accurate in anomaly detection. }
\label{fig3}
\end{figure}
%This approach has two major drawbacks. 
UCAD has two major drawbacks. 
% First, it compromises unstable results. 
% Specifically, the task identification of UCAD depends on the ViT which is initially pre-trained on ImageNet. 
% However, a distribution shift exists between ImageNet and real-world images, which can diminish the reliability of classification. 
% As shown in Fig.~\ref{fig:mismatch}, two typical mismatches in UCAD are presented due to task similarity and background similarity, respectively.
% Tab.~\ref{tab:accuracy} displays the classification accuracy across all categories in MVTec AD during the task identification phase of UCAD. 
% Notably, the leather's classification accuracy is significantly low, marked at only 50.81\%.
% Tab.~\ref{tab:pixel-leather} illustrates the performance degradation of UCAD on the leather category, highlighting the unreliability and cumulative task identification errors of UCAD's two-stage method~(shown in Fig.~\ref{fig:visual2}).
% In contrast, our method is task-free and directly detects anomalies from the input image, yielding more stable results.
First, UCAD demonstrates instability in its performance due to its reliance on task identification through feature matching with a pre-trained Vision Transformer (ViT). Since the ViT is trained on ImageNet, a substantial distribution shift exists between ImageNet and real-world industrial test images, rendering the feature-matching-based task identification process unreliable.  As illustrated  in Fig.~\ref{fig:mismatch}, task identification in UCAD is particularly affected by semantic similarities between tasks and the resemblance of foreground and background features across tasks. Tab.~\ref{tab:accuracy} presents the task identification accuracy across all categories in the MVTec AD dataset, highlighting significant challenges. For instance, the accuracy for the leather category is particularly low, at just 50.81\%, which severely impacts it's performance~(shown in Tab.~\ref{tab:pixel-leather}). As illustrated in Fig.~\ref{fig:visual2}, task identification errors often result in incorrect prompt selection, leading to complete detection failures and, consequently, unstable anomaly detection outcomes. In contrast, our end-to-end approach eliminates the need for task identification altogether. By directly detecting anomalies from input images, our method ensures more stable and reliable results, overcoming the limitations observed in UCAD.

\begin{table*}[!ht]
\centering
{\footnotesize
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{Pixel-level}} & \multicolumn{4}{c}{\textbf{Image-level}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& \multicolumn{2}{c}{\textbf{ACC} $\uparrow$} & \multicolumn{2}{c}{\textbf{FM} $\downarrow$} & \multicolumn{2}{c}{\textbf{ACC} $\uparrow$} & \multicolumn{2}{c}{\textbf{FM} $\downarrow$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
& \textbf{AUROC} & \textbf{AUPR} & \textbf{AUROC} & \textbf{AUPR} & \textbf{AUROC} & \textbf{AUPR} & \textbf{AUROC} & \textbf{AUPR} \\
\midrule
% \multicolumn{5}{l}{\textit{Incremental Anomaly Detection Methods}} \\
Baseline + L2P   & \underline{93.56} & \underline{42.66} & \underline{2.09} & \underline{2.14} &  \underline{91.86} & 95.76 & 0.73 &  0.31\\
Baseline + DualPrompt   & 92.79 & 41.32 & 2.83 & 9.63 & 91.81 & \underline{5.77} & 1.12 & 0.55 \\

Baseline + L2P + LwF & 93.28 & 41.77 & 2.58 & 2.88 &  91.69 & 95.38 & \textbf{0.57} &  0.68\\
Baseline + DualPrompt + LwF & 92.74 & 42.15 & 2.67 & 2.21 & 91.47 & 95.63 &1.02 & 0.58 \\
% Baseline + L2P + LwF &  &  &  &  &  &  & &  \\
Baseline + L2P + $\text{DER}^\#$ & 92.65 & 42.55 & 2.68 & 2.17 & 91.47 & 95.43 & 0.34 & \textbf{0.13}  \\
% Baseline + DualPrompt + LwF &  &  &  &  &  &  & &  \\
Baseline + DualPrompt + $\text{DER}^\#$ & 92.91 & 41.93 & 2.83 & 3.20 & 91.01 & 95.22 & 1.23& 0.92 \\
% Baseline + startPrompt + LwF &  &  &  &  &  &  & &  \\
% Baseline + $\text{DER}^\#$  &  &  &  &  &  &  & &  \\
\midrule
\textbf{ONER} (Ours) & \textbf{94.53} & \textbf{49.66} & \textbf{0.91} & \textbf{1.33} & \textbf{93.36} & \textbf{97.26} & \underline{0.59} & \underline{0.15} \\
\bottomrule
\end{tabular}}
\caption{Comparison with different incremental learning methods on the MVTec AD dataset ($N=15$) after training on the last subset. Bold and underline highlight the best and second-best results. The symbol (\#) denotes methods that replay original samples from previous tasks.}
%methods that use task-specific models.
\label{tab:mvtec-prompt}
\end{table*}


\begin{table*}[!t]
\centering
{\footnotesize
\begin{tabular}{lcccccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{Pixel-level}} & \multicolumn{4}{c}{\textbf{Image-level}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& \multicolumn{2}{c}{\textbf{ACC} $\uparrow$} & \multicolumn{2}{c}{\textbf{FM} $\downarrow$} & \multicolumn{2}{c}{\textbf{ACC} $\uparrow$} & \multicolumn{2}{c}{\textbf{FM} $\downarrow$} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
& \textbf{AUROC} & \textbf{AUPR} & \textbf{AUROC} & \textbf{AUPR} & \textbf{AUROC} & \textbf{AUPR} & \textbf{AUROC} & \textbf{AUPR} \\
\midrule
% \multicolumn{5}{l}{\textit{Incremental Anomaly Detection Methods}} \\
Baseline + L2P  & 84.04 & 19.01 & 8.49 & 8.81 & \underline{78.89} & \underline{82.95} & \textbf{2.46} & \textbf{1.91} \\
Baseline + DualPrompt   & 86.43 & 19.73 & 6.13 & 8.54 & 76.56 & 80.64 & 5.48& 4.54\\
Baseline + L2P + LwF & 84.28 & 17.93 & 7.02 & 9.63 & 74.70 & 79.38 & 6.75 & 5.75 \\
Baseline + DualPrompt + LwF & 87.74 & 18.88 & 5.19 & 9.21 & 76.95 & 80.48 & 5.11& 4.57 \\

% Baseline + L2P + LwF &  &  &  &  &  &  & &  \\
Baseline + L2P + $\text{DER}^\#$ & 85.73 & 19.83 & 6.27 & 8.33 & 75.01 &  79.56 &  6.09 &  5.1\\
% Baseline + DualPrompt + LwF &  &  &  &  &  &  & &  \\
Baseline + DualPrompt + $\text{DER}^\#$ & \underline{88.84} & \underline{20.24} & \underline{2.71} & \underline{6.94} & 77.62 & 82.22 & 4.41 & 2.81 \\
% Baseline + startPrompt + LwF &  &  &  &  &  &  & &  \\


% Baseline + $\text{DER}^\#$  &  &  &  &  &  &  & &  \\
\midrule
\textbf{ONER} (Ours)& \textbf{90.58} & \textbf{27.87} & \textbf{2.39} & \textbf{1.82} & \textbf{83.14} & \textbf{86.61} & \underline{3.88} & \underline{2.70} \\
\bottomrule
\end{tabular}}
\caption{Comparison with different incremental learning methods on the VisA dataset ($N=12$) after training on the last subset. Bold and underline highlight the best and second-best results. The symbol (\#) denotes methods that replay original samples from previous tasks.}
%methods that use task-specific models.
\label{tab:visa-prompt}

\end{table*}
The second drawback of UCAD concerns testing efficiency and storage requirements. UCAD requires multiple comparisons—one for each task—to identify the task associated with the input image, followed by a final comparison to generate the result. In contrast, our method only requires a single comparison, enhancing its testing efficiency.
Regarding storage, UCAD needs to store task-specific features with a shape of $(2,196,1024)$, which includes both key and knowledge features for each new task. Our method, however, stores features with a shape of $(197,768)$, encompassing image-level prototypes (shape $(1,768)$)  and pixel-level prototypes (shape $(196,768)$), making our approach much more storage-efficient.

In summary, our method surpasses UCAD in several key areas: achieving higher accuracy with lower forgetting, enhanced stability, improved testing efficiency, and reduced storage requirements. By eliminating the need for task identification during inference, our approach avoids the cumulative errors inherent in UCAD, ensuring more reliable and stable results. Furthermore, our method optimizes testing efficiency by streamlining the process and minimizes storage demands, making it a more efficient and robust solution for incremental anomaly detection.

\section{Additional details}
\subsection{Details for evaluation metrics}
\textbf{Forgetting Measure (FM)} evaluates the model's resistance to catastrophic forgetting in a class-incremental setting. This metric assesses how well the model retains knowledge of previously learned tasks as new tasks are introduced. Lower FM values indicate better retention of prior knowledge and thus more stable learning.

Since there are two modes during testing including the end-to-end and staged approach, the calculation of FM varies for each mode.

\begin{itemize}

\item \textbf{End-to-end}: In this mode, a unified model is utilized for all tasks, which faces the issue of catastrophic forgetting. Therefore, the FM for the end-to-end approach is calculated as follows:
  \begin{equation}
  FM_{e}=\frac{1}{N-1}\sum_{i=1}^{N-1}\max_{j\in\{1,~\dots,~N-1\}}(\text{M}_{j,i}-\text{M}_{N,i}) ,
  \end{equation}
  where \( N \) is the total number of tasks, \( \text{M}_{j,i} \) represents the evaluation metric for task \( i \) measured after learning task \( j \), and \( \text{M}_{N,i} \) is the evaluation metric for task \( i \) measured after learning all tasks.
  
\item \textbf{Staged Approach}: 
Unlike end-to-end mode, staged approach first identifies each task via a classifier and subsequently applies a task-specific model for anomaly detection.
However, the effectiveness of the staged approach is significantly dependent on the accuracy of task identification in the first stage.

To this end, the FM for the staged approach is calculated as:
  \begin{equation}
  FM_{s} = \frac{1}{N}\sum_{i=1}^{N}\left(\text{M}_{\text{known},i} - \text{M}_{\text{pred},i} \right),
  \end{equation}
  where \( \text{M}_{\text{known},i} \) is the evaluation metric assuming the true class of the input image is known, and \( \text{M}_{\text{pred},i} \) is the evaluation metric when the class of the input image is predicted before anomaly detection.
\end{itemize}

These FMs help us understand the robustness of our model in retaining previously learned information and adapting to new tasks, ensuring a comprehensive evaluation of performance in class-incremental learning scenarios.

\subsection{Details for incremental classifier}
 \textbf{Incremental Classifier-based}: This strategy involves training an incremental classifier and task-specific models. The classifier is based on DER \cite{buzzega2020dark} and manages new classes, similar to UCAD’s task identification stage. Each new task requires a separate model, and the class-incremental classifier maintains categorization. We use a pre-trained ResNet18 model with selective freezing of the backbone’s final layer and training of the fully connected (fc) layer, employing SGD with a learning rate of 0.0005, a batch size of 10, and 25 epochs. For each task, five samples and their logits are saved for future training. This method achieved 69.45\% accuracy on the MVTec AD dataset ($N=15$) and 80.53\% on the VisA dataset ($N=12$).
 % \begin{table}[t]
% \centering
% \small
% % {\footnotesize
% \begin{tabular}{lcc}
% \toprule
% Method & Learnable Parameters & Epochs \\
% \midrule
% DRAEM~\textcolor{gray}{\tiny [ICCV21]} & 97.42M & 300 \\
% % GLAD~\textcolor{gray}{\tiny [ECCV24]} & 859.52M  & 280\\
% BGAD~\textcolor{gray}{\tiny [CVPR23]} & 3.39M & 100 \\
% % STPM~\textcolor{gray}{\tiny [BMVC21]} & & \\
% % SimpleNet~\textcolor{gray}{\tiny [CVPR23]} & 3.94M & 160 \\
% % \midrule
% DRAEM-Replay & 97.42M & 300\\
% BGAD-Replay & 3.39M & 100\\
% DRAEM-CLS* & (97.42+8.40)M & 300+10\\
% BGAD-CLS* & (3.39+8.40)M & 100+10\\
% % \midrule
% \hline


% CAD~\textcolor{gray}{\tiny [ACM MM23]} & 85.21M & 50 \\
% IUF~\textcolor{gray}{\tiny [ECCV24]} & 9.11M & 200 \\
% UCAD*~\textcolor{gray}{\tiny [AAAI24]} & 0.021M & 25 \\

% % \midrule
% \hline
% \textbf{ONER} (Ours) & \textbf{0.019M} & \textbf{5} \\
% \bottomrule
% \end{tabular}
% \caption{Statistics of learnable parameters and training epochs per task for different methods on the MVTec AD dataset.}
% \label{tab:parameter_epochs_statistics}
% \end{table}
\section{Additional experiments}
\subsection{Additional qualitative study}
Fig.~\ref{fig3} illustrates the substantial performance decline caused by task identification inaccuracies within a two-stage approach, highlighting its unreliability.
In contrast, our method directly processes input images, resulting in more stable and dependable detection outcomes.
\subsection{Experiments with different prompt-tuning method}
We enhance our baseline with two prompt-tuning methods: Learning to Prompt~(L2P)~\cite{Wang_Zhang_Lee_Zhang_Sun_Ren_Su_Perot_Dy_Pfister_2022} and DualPrompt~\cite{wang2022dualprompt}. 
Additionally, we further optimize these configurations by introducing LwF~\cite{DBLP:conf/eccv/LiH16}.
%, resulting in versions of our baseline enhanced with L2P and LwF, and DualPrompt and LwF.
% We also optimize the prompt structure by integrating the latest Visual Fourier Prompt Tuning (VFPT)~\cite{zeng2024visual}, leading to two further configurations: one with L2P and VFPT, and the other with DualPrompt and VFPT.
Furthermore, We also extend these configurations by introducing Dark Experience Replay~(DER)~\cite{buzzega2020dark}, which rehearses 5 images per tasks.
%, resulting in versions of our baseline enhanced with L2P and DER, and DualPrompt and DER.
It is important to highlight that we use $\mathcal{L}_{\text{TSC}}$ as the core loss function for prompt optimization. As demonstrated in Tables~\ref{tab:mvtec-prompt} -~\ref{tab:visa-prompt}, our method outperforms other incremental learning approaches.
\subsection{Experiments with incremental orders}
In the main paper, we follow UCAD's approach by organizing the incremental learning sequence alphabetically by category. To further validate our method's robustness, we conduct additional experiments using a randomly shuffled incremental order. As shown in Tab.~\ref{tab:order-visa} - \ref{tab:order-mvtec}, our method maintains consistent performance regardless of the sequence, indicating the robustness of the method.

\begin{table}[h]
% \centering
{\footnotesize
\begin{tabular}{lcccc}
\toprule
\textbf{Incremental Order} & \multicolumn{2}{c}{\textbf{Image-level}} & \multicolumn{2}{c}{\textbf{Pixel-level}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 &   \textbf{AUROC} & \textbf{AUPR} & \textbf{AUROC} & \textbf{AUPR} \\
\midrule
Alphabetical (Asc) & 83.14 & 86.61 & 90.58 & 27.87 \\
\midrule
% Alphabetical (Desc) & 80.08 & 83.76 & 84.39 & 20.90 \\
% \midrule
Random Order 1 &  83.27 & 86.63 & 90.74 & 25.88 \\
\midrule
Random Order 2 &  82.94 & 86.08 & 90.29 & 27.52 \\
\midrule
Random Order 3 &  81.99 & 85.71 & 90.14 & 26.04 \\
\bottomrule
\end{tabular}}
\caption{Evaluation of performance metrics on the VisA dataset across various incremental orders for our method.}
\label{tab:order-visa}

\end{table}

\begin{table}[h]
% \centering
{\footnotesize
\begin{tabular}{lcccc}
\toprule
\textbf{Incremental Order} & \multicolumn{2}{c}{\textbf{Image-level}} & \multicolumn{2}{c}{\textbf{Pixel-level}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 &   \textbf{AUROC} & \textbf{AUPR} & \textbf{AUROC} & \textbf{AUPR} \\
\midrule
Alphabetical (Asc) & 93.36 & 97.26 & 94.53 & 49.66 \\
\midrule
Random Order 1 & 93.94 & 97.29 & 93.69 & 48.90 \\
\midrule
Random Order 2 &  93.30 & 97.10 & 94.43 & 49.05 \\
\midrule
% Random Order 2 &  93.25 & 96.83 & 93.91 & 48.42 \\
% \midrule
Random Order 3 &  93.10 & 96.82 & 94.77 & 48.82 \\

\bottomrule
\end{tabular}}
\caption{Evaluation of performance metrics on the MVTec AD dataset across various incremental orders for our method.}
\label{tab:order-mvtec}

\end{table}

% \begin{table}[h]
% \centering
% {\footnotesize
% \begin{tabular}{lcccc}
% \toprule
% $L_p$ & \multicolumn{2}{c}{\textbf{Image-level}} & \multicolumn{2}{c}{\textbf{Pixel-level}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%  &   \textbf{AUROC} & \textbf{AUPR} & \textbf{AUROC} & \textbf{AUPR} \\
% \midrule
% \midrule
% % 45 & 18 &  &   &  &   \\
% % \midrule
% % 45 & 6 &   &   &  & \\
% % \midrule
% % 30 & 12 &  &   &  &    \\
% % \midrule
% 18 & \textbf{93.44}  &  \underline{97.12} & 93.61 & \underline{48.94}\\
% \midrule
% 12 & 93.01  &  96.87 & \underline{94.16} & 48.71\\
% \midrule
% % Random Order 2 &  93.25 & 96.83 & 93.91 & 48.42 \\
% % \midrule
%  6 &  \underline{93.36} & \textbf{97.26} & \textbf{94.53} & \textbf{49.66} \\

% \bottomrule
% \end{tabular}}
% \caption{Ablation study of  $L_p$ on the MVTec AD dataset.}
% \label{tab:htyper-mvtec}

% \end{table}

% \begin{table}[!tp]
% % \centering
% {\footnotesize
% \begin{tabular}{lcccc}
% \toprule
% \textbf{inserted layers} & \multicolumn{2}{c}{\textbf{Image-level}} & \multicolumn{2}{c}{\textbf{Pixel-level}} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
%  &   \textbf{AUROC} & \textbf{AUPR} & \textbf{AUROC} & \textbf{AUPR} \\
% \midrule
% $[0]$ & \underline{93.78}  & \underline{97.48} & 93.94 & 48.53\\
% \midrule
% $[5]$ & 92.82  & 96.92 & 93.87 & 48.29\\
% \midrule
% $[0,1,2]$ & 93.64  & 97.25 & \underline{93.99} & 48.15\\
% \midrule
% $[0,1,11]$ & \textbf{94.24}  & \textbf{97.61} & 93.94 &  48.28\\
% \midrule
% $[4, 5,6]$ & 93.29  & 97.17 & 93.67 &  48.14\\
% \midrule
% $[5,6,7]$ & 93.70  & 97.38 & 93.79 &  \underline{48.65}\\
% \midrule
% $[0,5,11]$ &  93.36 & 97.26 & \textbf{94.53} & \textbf{49.66} \\

% \bottomrule
% \end{tabular}}
% \caption{Ablation study of different layers where prompts are inserted on the MVTec AD dataset for our method.}
% \label{tab:prompt-inserts}

% \end{table}

\end{appendices}
